End-To-End Clinical Trial Matching with Large Language Models

Matching cancer patients to clinical trials is essential for advancing treatment and patient care. However, the inconsistent format of medical free text documents and complex trial eligibility criteria make this process extremely challenging and time-consuming for physicians. We investigated whether the entire trial matching process - from identifying relevant trials among 105,600 oncology-related clinical trials on clinicaltrials.gov to generating criterion-level eligibility matches - could be automated using Large Language Models (LLMs). Using GPT-4o and a set of 51 synthetic Electronic Health Records (EHRs), we demonstrate that our approach identifies relevant candidate trials in 93.3% of cases and achieves a preliminary accuracy of 88.0% when matching patient-level information at the criterion level against a baseline defined by human experts. Utilizing LLM feedback reveals that 39.3% criteria that were initially considered incorrect are either ambiguous or inaccurately annotated, leading to a total model accuracy of 92.7% after refining our human baseline. In summary, we present an end-to-end pipeline for clinical trial matching using LLMs, demonstrating high precision in screening and matching trials to individual patients, even outperforming the performance of qualified medical doctors. Our fully end-to-end pipeline can operate autonomously or with human supervision and is not restricted to oncology, offering a scalable solution for enhancing patient-trial matching in real-world settings.

==> Manuscript/search_trials_location.tex <==
\begin{longtable}{@{}l|p{2.4cm}|p{2.4cm}|p{2.4cm}|p{2.4cm}@{}}

\caption*{{\Large Table 1: }}\\
\toprule
\multicolumn{1}{c|}{\textbf{No.}} & \multicolumn{1}{c|}{\textbf{Prefiltered}} & \multicolumn{1}{c|}{\textbf{Retrieved}} & \multicolumn{1}{c|}{\textbf{Final}} & \multicolumn{1}{c}{\textbf{Reranked}} \\
\midrule
\endfirsthead
\toprule
\multicolumn{1}{c|}{\textbf{No.}} & \multicolumn{1}{c|}{\textbf{Prefiltered}} & \multicolumn{1}{c|}{\textbf{Retrieved}} & \multicolumn{1}{c|}{\textbf{Final}} & \multicolumn{1}{c}{\textbf{Reranked}} \\
\midrule
\endhead
\midrule

\endfoot
\bottomrule
\endlastfoot


1 & \xmark\phantom{ab}(51/512) & \xmark\phantom{ab}(31/183) & \cmark\phantom{ab}\textbf{(4/16)} & \cmark\phantom{ab}(8/16) \\
2 & \xmark\phantom{ab}(1170/2903) & \xmark\phantom{ab}(26/282) & \cmark\phantom{ab}\textbf{(7/37)} & \xmark\phantom{ab}(28/37) \\
3 & \xmark\phantom{ab}(315/830) & \cmark\phantom{ab}\textbf{(2/228)} & \cmark\phantom{ab}\textbf{(2/20)} & \xmark\phantom{ab}(14/20) \\
4 & \xmark\phantom{ab}(272/440) & \xmark\phantom{ab}(21/190) & \cmark\phantom{ab}\textbf{(5/8)} & \cmark\phantom{ab}(6/8) \\
5 & \xmark\phantom{ab}(47/125) & \cmark\phantom{ab}\textbf{(1/119)} & \cmark\phantom{ab}\textbf{(1/1)} & \cmark\phantom{ab}\textbf{(1/1)} \\
6 & \xmark\phantom{ab}(60/805) & \xmark\phantom{ab}(12/182) & \cmark\phantom{ab}\textbf{(4/26)} & \cmark\phantom{ab}(9/26) \\
7 & \xmark\phantom{ab}(15/170) & \cmark\phantom{ab}\textbf{(2/144)} & \cmark\phantom{ab}(3/29) & \xmark\phantom{ab}(22/29) \\
8 & \xmark\phantom{ab}(13/181) & \cmark\phantom{ab}(8/151) & \cmark\phantom{ab}\textbf{(6/34)} & \xmark\phantom{ab}(28/34) \\
9 & \cmark\phantom{ab}\textbf{(4/227)} & \cmark\phantom{ab}(10/159) & \cmark\phantom{ab}(6/29) & \xmark\phantom{ab}(15/29) \\
10 & \xmark\phantom{ab}(19/144) & \cmark\phantom{ab}\textbf{(4/136)} & \cmark\phantom{ab}(8/28) & \xmark\phantom{ab}(23/28) \\
11 & \xmark\phantom{ab}(70/109) & \xmark\phantom{ab}(50/106) & \xmark\phantom{ab}(28/32) & \cmark\phantom{ab}\textbf{(9/32)} \\
12 & \xmark\phantom{ab}(28/75) & \cmark\phantom{ab}\textbf{(1/75)} & \cmark\phantom{ab}\textbf{(1/33)} & \cmark\phantom{ab}(4/33) \\
13 & \cmark\phantom{ab}(7/18) & \cmark\phantom{ab}(10/18) & \cmark\phantom{ab}(4/6) & \cmark\phantom{ab}\textbf{(3/6)} \\
14 & \xmark\phantom{ab}(17/18) & \cmark\phantom{ab}(4/18) & \cmark\phantom{ab}\textbf{(2/18)} & \cmark\phantom{ab}(3/18) \\
15 & \cmark\phantom{ab}\textbf{(4/42)} & \xmark\phantom{ab}(11/42) & \cmark\phantom{ab}(5/24) & \cmark\phantom{ab}(8/24) \\

\noalign{\vskip 0.2mm} % Add vertical space before the summary row
\midrule
\multicolumn{1}{c|}{$\sum$} & \multicolumn{1}{c|}{3/15} & \multicolumn{1}{c|}{9/15} & \multicolumn{1}{c|}{\textbf{14/15}} & \multicolumn{1}{c}{9/15} \\
\bottomrule
\end{longtable}
